Client-Centric Federated Adaptive Optimization

Federated Learning (FL) is a distributed learning paradigm where clients collaboratively train a model while keeping their own data private. With an increasing scale of clients and models, FL encounters two key challenges, client drift due to a high degree of statistical/system heterogeneity, and lack of adaptivity. However, most existing FL research is based on unrealistic assumptions that virtually ignore system heterogeneity. In this paper, we propose Client-Centric Federated Adaptive Optimization, which is a class of novel federated adaptive optimization approaches. We enable several features in this framework such as arbitrary client participation, asynchronous server aggregation, and heterogeneous local computing, which are ubiquitous in real-world FL systems but are missed in most existing works. We provide a rigorous convergence analysis of our proposed framework for general nonconvex objectives, which is shown to converge with the best-known rate. Extensive experiments show that our approaches consistently outperform the baseline by a large margin across benchmarks.

==> subfiles/algorithm_draft.tex <==
\section{Client-Centric Federated Adaptive Optimization}
\label{sec:client-centric}

In this section, we first introduce the key limitations of existing FL algorithms, which requires heavy server-client coordination and ignores system heterogeneity in Section \ref{subsec:server-centric-limitation}. In light of the limitations, We then introduce our proposed algorithm Client-Centric Federated Adaptive Optimization in Section \ref{subsec:proposed_alg}.

\subsection{Limitations of Server-Centric FL}
\label{subsec:server-centric-limitation}


All proposed federated learning algorithms rely on a key assumption that may rarely hold in real world deployment, that is,

\begin{tcolorbox}
\begin{center}
\vspace{-0.05in}
\textbf{ At a given round, all clients update with the same global model and they conduct identical number of local computations. }
\vspace{-0.05in}
\end{center}
\end{tcolorbox}

More formally, we extract the local computation of previous federated learning paradigms in Algorithm \ref{alg:local_computation}.


\begin{algorithm2e}
\SetAlgoVlined
\KwIn{
\textbf{local} learning rate $\eta_l$, \textbf{local} updating number $K$\;
}
\SetAlgoLined
At round $t$, uniformly sample a subset $\mathcal{S}_t$ of clients
    
Server sends $x_t$ to subset $\mathcal{S}_t$ of clients
    
\For{ each client  $i\in \mathcal{S}_t$}
{
    Initialize $x_{t,0}^i\gets x_t$
    
    \For{$k\in\{0,1,...,K-1\}$}
    {
    Randomly sample a batch $\xi_{t,k}^i$
    
    Compute $g_{t,k}^i=\nabla f_i(x_{t,k}^i, \xi_{t,k}^i)$
    
    Update $x_{t,k+1}^i=x_{t,k}^i-\eta_l g_{t,k}^i$
    }
    $\Delta_t^i=x_t-x_{t,K}^i$
    }
    
\caption{Local Computation in Server Centric Federated Learning}
\label{alg:local_computation}
\end{algorithm2e}

We could observe the following settings have been assumed in all previous algorithms,

\begin{itemize}[leftmargin=*]
    \item \textbf{(Homogeneous Local Updates)} All participating would do local gradient descent for $K$ steps.
    \item \textbf{(Uniform Client Participation)} Each client would participate in a given communication round uniformly according to a given distribution that is independent across rounds.
    \item \textbf{(Synchronous Local Clients)} All participating clients always initialize at $x_t$, i.e., the global model at current timestamp.
\end{itemize}

For a simplified characterization of real world scenarios and appealing theoretical convergence guarantee, these three assumptions have been widely adopted in most existing federated learning literature, e.g., \cite{McMahan2017FedAvg,Hsu2019MeasuringTE,Li20FedProx,karimireddy2020scaffold,reddi2020adaptive,acar2021feddyn,wang22adaptive}.

However, we would like to argue that any of these assumptions rarely holds in reality, especially considering that federated learning typically takes thousands of communication rounds to converge in large-scale cross-device deployments, it is impossible to ensure these assumptions hold throughout the whole process,

\begin{itemize}[leftmargin=*]
    \item \textbf{(Heterogeneous Client Capability)} Each of the clients may have widely different computational capability, and faster clients are able to carry out more local computations than slower clients. Requesting identical local updates would straggle the training and incur unnecessary energy waste.
    \item \textbf{(Unpredictable Client Availability)} The clients have diversified availability due to various participation constraints, e.g. unstable network connection, low battery level, or participation willingness \citep{Kairouz21AdvancesProblems,Li2019Fed_Survey}. Therefore, each client typically participates
    in a given communication round purely dependent on its own condition and the decision is completely unpredictable to the server. The uniform participation assumption is over-simplifying this process.
    \item \textbf{(Asynchronous Local Model)} Due to the random nature of client participation and capability, the server typically does not wait until the slowest participating client completes local computation, and would instead start the next round whenever a sufficient number of clients respond. The rest of the clients would participate in a future round when they finish and decide to respond. Though more efficient than its synchronous counterpart, clients may be computing based on global model up to a random delay $\tau_{t,i}$, i.e., calculating local gradients based on global model $x_{t-\tau_{t,i}}$ instead of $x_t$, in this asynchronous mechanism.
\end{itemize}

Therefore, due to clients' system heterogeneity in availability and capability, the applicability of the key assumption and the theoretical analysis derived based on that is questionable. Traditionally, most works that recognize client heterogeneity focus explicitly on data heterogeneity \citep{Li2020Fed-Non-IID,yang2021achieving}, i.e. the local data distribution distinguishes with each other, while in reality the system heterogeneity is as ubiquitous as data heterogeneity and largely remains unanswered.

The existing works that are dedicated to studying system heterogeneity can be mainly categorized into the following groups,

\begin{itemize}[leftmargin=*]
    \item Heterogeneous local computing but synchronous aggregation. \cite{Wang20FedNova} is probably the first work to show heterogeneous number of local updates results in the global model converges to a mismatched optimum which can be arbitrarily away from the true optimum and proposes an effective remedy FedNova to correct the mismatch. \cite{Ruan2021FlexibleParticipation} analyzes the impact of a more flexible mechanism where clients may be inactive, return incomplete updates, depart early or arrive late. \cite{Basu19Qsparse-Local-SGD} considers how model compression works with different number of local updates \footnote{Though the authors call the proposed model 'asynchronous', the asynchrony refers to that updates occur after different number of local iterations but the local iterations are synchronous with respect to the global clock. However, 'asynchronous' in our context refers to local iterations are asynchronous with respect to the global clock, which is more challenging to analyze.}. \cite{Avdiukhin21arbitrarycommunication} focuses on a similar setting and studies the upper bound of distances between two consecutive communications to reduce communication times as much as possible. Their theoretical analysis relies on bounded gradient assumption.
    \item Flexible participation scheme but synchronous aggregation. There are mainly two line of works in this class. The first line focuses on the issue of intermittent client availability, \cite{Yan2020DistributedClient} (FedLaAvg) and \cite{gu2021arbitraryunavailable} (MIFA) both allow clients to participate arbitrarily. However, the proposed approach still requires all devices have to respond in the first round. Moreover, the theoretical analysis of FedLaAvg requires bounded gradient assumption while MIFA requires a Lipschitz Hessian assumption, which are too stringent and unnecessary. \cite{wang2022arbitraryparticipation} systematically studies various participation patterns and which one of them guarantees convergences and whether the rate of convergence matches idealized participation scheme. However, their work considers synchronous aggregation and only the case of vanilla FedAvg. The second line concentrates on biased client selection \citep{Nishio2018ClientSelection, Chen2020ClientSampling, cho22biased_selection}. Most works study the biased sampling strategy in which the probability a client is sampled is related to its local loss to accelerate training \citep{Goetz2019ActiveFL,Ribero2020clientsampling}, which is inspired by similar strategy in centric computing \citep{Salehi2017BanditSampling,Jiang2019Local_Loss,shah20local_loss,Katharopoulos2018ImportanceSampling}. This line of works is less related to our proposed research.
    \item Asynchronous aggregation. This line of research is cloest related to ours. However, though asynchrony has been a decade-long topic in traditional distributed computing \citep{Zhang2014DeepElasticAvg,Lian15Asynchronous,Zheng17ASGD}, it has received very limited attention in federated learning. \cite{Xie2019AsynchronousFO} proposes FedAsync in which the server immediately updates the global model whenever it receives a single local model. Their theoretical analysis only applies to convex objective function which is not applicable to deep learning. Moreover, this proposal has negative implication in privacy, as it no longer hides one single update in an aggregate, which is one of the most important points to use FL in the first place. In light of this, \cite{Nguyen2021FedBuff} proposes FedBuff, in which a global update is triggered when the server receives $m$ local updates, where $m$ is a pre-specified hyperparameter. By maintaining a size $m$ buffer, FedBuff could secure the identity of each local update and is empirically faster than FedAsync. However, it does not consider the heterogeneous local computing and does not provide a convergence rate that shows the dependency on $m$. \cite{Yang2021AnarchicFL} proposes anarchic FL in which the clients are free to determine how much local computation to conduct and the asynchronous communication is in the same fashion as FedBuff. However, \cite{Yang2021AnarchicFL} only considers the case of vanilla FedAvg.
\end{itemize}

\begin{algorithm2e}
\SetAlgoVlined
\KwIn{\\
Number of clients $n$, objective function $f(x)=\frac{1}{n}\sum_{i=1}^n f_i(x)$, initialization $x_0$\; 
Number of communication rounds $T$, \textbf{local} learning rate $\eta_l$\;
Triplets of (\textbf{global} learning rate, momentum factor, instant discount factor) $\{\eta,\beta,\nu\}$;}
\SetAlgoLined
\For{$t\in\{0,1,...,T-1\}$}
{   
    \textcolor{red}{\underline{\textbf{At Each Worker (Concurrently)}}}

    Once decided to participate in the training, retrieve $x_\mu$ from the server and its timestamp, set $x_{\mu,0}^i=x_\mu$.

    Self-select a number of local steps $K_{t,i}$, which can be time-varying and device-dependent.

    \For{$k\in\{0,1,...,K_{t,i}-1\}$}
    {
    Randomly sample a batch $\xi_{\mu,k}^i$
    
    Compute $g_{\mu,k}^i=\nabla f_i(x_{\mu,k}^i; \xi_{\mu,k}^i)$
    
    Update $x_{\mu,k+1}^i=x_{\mu,k}^i-\eta_l g_{\mu,k}^i$
    }
    $\Delta_\mu^i=x_\mu-x_{\mu,K_{t,i}}^i$

    Normalize and send $\Delta_\mu^i=\frac{\Delta_\mu^i}{K_{t,i}}$
    

    \textcolor{red}{\underline{\textbf{At Server (Concurrently)}}}
    

    Collect $m$ local updates $\{\Delta_{t-\tau_{t,i}}^i, i\in\mathcal{M}_t\}$ returned from the workers to form set $\mathcal{S}_t$, where $\tau_{t,i}$ represents the random delay of the worker $i$'s local update, $i\in\mathcal{S}_t$

    Aggregate and update: $\Delta_t=\frac{1}{m}\sum_{i\in \mathcal{S}_t}\Delta_{t-\tau_{t,i}}^i$

    \colorbox{yellow}{Update $x_{t+1}=x_t-\eta \Delta_t$}
    
    \colorbox{green}{$d_{t+1}=(1-\beta)\Delta_{t}+\beta d_{t}$, $h_{t+1}=(1-\nu)\Delta_{t}+\nu d_{t+1}$}

    \colorbox{green}{Update $x_{t+1}=x_t-\eta h_{t+1}$}

    \colorbox{magenta}{$d_{t+1}=(1-\beta)\Delta_{t}+\beta d_{t}$, $v_{t+1}=(1-\gamma)\Delta^2_{t}+\gamma v_{t}$}

    \colorbox{magenta}{$\hat{v}_{t+1}=\max(\hat{v}_{t},v_{t+1},\epsilon)$}

    \colorbox{magenta}{Update $x_{t+1}=x_t-\eta \frac{d_{t+1}}{\sqrt{\hat{v}_{t+1}}}$}

}
return $x_T$
\caption{\colorbox{yellow}{Autonomous FedAvg} \colorbox{green}{Autonomous FedGM} \colorbox{magenta}{Autonomous FedAMS}}
\label{alg:autonomous_fed_algs}
\end{algorithm2e}

\subsection{Proposed Algorithm: Client-Centric Federated Adaptive Optimization}
\label{subsec:proposed_alg}

In light of the limitations of related works, we aim to propose a general framework that enables all three features, i.e. heterogeneous local computing, asynchronous aggregation, and flexible client participation. Motivated by the compelling empirical performances from federated general momentum, we go one step further than vanilla FedAvg and integrate the general momentum in this autonomous federated learning framework. The pseudocode for Autonomous FedAvg and Autonomous FedGM is given in Algorithm \ref{alg:autonomous_fed_algs}.

Specifically, in Autonomous FedAvg, the client decides when to participate in the training, and idling between two consecutive rounds of participation or even unavailable throughout the whole process are both allowed, which characterizes realistic scenarios in cross-device FL. Once it decides to participate at round $t$, it retrieves current global model $x_\mu$ from the server and initializes $x_{\mu,0}^i=x_\mu$ locally, and conduct $K_{t,i}$ local steps to update from $x_{\mu,0}^i$ to $x^i_{\mu,K_{t,i}}$. Note in vanilla FedAvg, $K_{t,i}=K$ for any $i$ and $t$. In contrast, we allow maximum flexibility in our framework, $K_{t,i}$ can be time-varying and device dependent. The client then normalizes the model update by $K_{t,i}$, i.e. $\Delta_\mu^i=\frac{x_{\mu,0}^i-x_{\mu,K_{t,i}}^i}{K_{t,i}}$, to avoid model biased towards clients with more local updates. In the meantime, the server collects the model updates from the clients. As every client may participate in training at a different round, the collected model update $\Delta_{t-\tau_{t,i}}^i$ may be from a historic timestamp, i.e. $\tau_{t,i}$ from current time $t$. Our framework subsumes synchronous aggregation as a special example if we set the delay $\tau_{t,i}=0$ for any $i$ and $t$. The server triggers global update whenever it collects $m$ model updates and we denote the set of $m$ responsive clients as $\mathcal{S}_t$. The global update is same as vanilla FedAvg, i.e. $x_{t+1}=x_t-\eta \frac{1}{m}\sum_{i\in \mathcal{S}_t}\Delta_{t-\tau_{t,i}}^i$. Note that this process is concurrent with clients, i.e., the global update happens whenever $m$ model updates are collected, regardless of whether there are still some clients conducting local computation, thus ensuring there is no system locking or straggler.

In summary, our framework has the following few features,

\begin{itemize}[leftmargin=*]
    \item Global update happens simultaneously with local update, which avoids slow clients slowing down training.
    \item Client participates whenever it intends to, and can also self-determine a time-varying and device-dependent number of local updates $K_{t,i}$. 
    \item Global update at round $t$ can work with local model updates from historic timestamps $t-\tau_{t,i}$.
\end{itemize}

In Autonomous FedGM, we enable server momentum to leverage its two unique advantages, i.e. alleviating client drift and accelerating convergence. We still employ the general framework of general momentum to subsume a large class of momentum schemes as special examples. Autonomous FedAvg and Autonomous FedGM will recover FedAvg and FedGM, i.e. Algorithm \ref{alg:fed_avg_fed_gm}, if we set $K_{t,i}=K$ and $\tau_{t,i}=0$ for any $i$ and $t$. Please note that varying $K_{t,i}$ and nonzero $\tau_{t,i}$ bring nontrivial extra complexity to the theoretical analysis as can be seen in our proof.



\begin{algorithm2e}
\SetAlgoVlined
\KwIn{\\
Number of clients $m$, objective function $\mathcal{F}(x)=\frac{1}{m}\Sigma_{i=1}^m f_i(x)$\; 
Number of communication rounds $T$, \textbf{local} learning rate $\eta_l$, \textbf{local} updating number $K$\;
Initialization $x_0$, \textbf{global} learning rate $\eta$, $\beta_1$, $\beta_2$, $\epsilon$;}
\SetAlgoLined
\For{$t\in\{0,1,...,T-1\}$}
{   
    Randomly sample a subset $S_t$ of clients\;
    
    Server send $x_t$ to subset $S_t$ of clients\;
    
    \For{each client $i\in S_t$}
    {
    Initialize $x_{t,0}^i\gets x_t$\;
    
    \For{$k\in\{0,1,...,K-1\}$}
    {
    Randomly sample a batch $\xi_{t,k}^i$\;
    Compute $g_{t,k}^i=\nabla f_i(x_{t,k}^i\;\xi_{t,k}^i)$\;
    Update $x_{t,k+1}^i=x_{t,k}^i-\eta_l g_{t,k}^i$\;
    }
    $\Delta_t^i=x_t-x_{t,K}^i$\;
    }
    
    Server aggregates $\Delta_t=\frac{1}{\lvert S_t\rvert}\Sigma_{i\in S_t}\Delta_t^i$\;
    $m_{t}=(1-\beta_1)\Delta_{t}+\beta_1 m_{t-1}$\;
    \colorbox{magenta}{$v_{t}=v_{t-1}+\Delta_{t}^2$}
    
    \colorbox{red}{$v_{t}=(1-\beta_2)\Delta_{t}^2+\beta_2 v_{t-1}$}
    
    \colorbox{yellow}{$v_{t}=(1-\beta_2)\Delta_{t}^2+\beta_2 v_{t-1}$}
    
    \colorbox{yellow}{$\hat{v}_{t}= \max(\hat{v}_{t-1},v_{t})$}
    
    Update $x_{t+1}=x_t-\eta \frac{m_t}{\sqrt{\hat{v}_t}+\epsilon}$\;
}
return $x_T$
\caption{Federated Adaptive Optimization, \colorbox{magenta}{FedAdagrad}, \colorbox{red}{FedAdam}, \citep{reddi2020adaptive} \colorbox{yellow}{FedAMSGrad} \citep{wang22adaptive}}
\label{fed_adaptive_alg}
\end{algorithm2e}


In centric computing environment, SGD is known to suffer to convergence when encountering heavy-tail stochastic gradient noise distributions, which is ubiquitous in large-scale model training \citealp{devlin2018bert,dosovitskiy2021VIT}. Adaptive optimizers, which adaptively adjust the learning rate on a per-feature basis, is shown to converge much faster than SGD in many applications. The volume of adaptive optimization methods makes it very difficult to exhaustively list them here, but they share similar design, i.e. scale coordinates of the gradient by square roots of some form of averaging of the squared coordinates \citep{reddi18adam_convergence}. Most representative optimizers in this class include AdaGrad \citep{duchi11adaptive}, Adam \citep{Kingma2015AdamAM}, and their variants e.g.  RMSProp \citep{tieleman2012rmsprop}, AdaDelta \citep{Zeiler2012ADADELTAAA}, AdaBound \citep{luo2018adabound}, AMSGrad \citep{reddi18adam_convergence}, AdaBelief \citep{zhuang2020adabelief}, RAdam \citep{Liu2020RAdam}.

\cite{reddi2020adaptive} is probably the first work to study the adaptive server optimization in federated learning context. Specifically, \cite{reddi2020adaptive} proposes a number of federated adaptive optimizers, e.g. FedAdam/FedYogi/FedADAGrad, whose pseudocode is in Algorithm \ref{fed_adaptive_alg}. They basically replace the original FedAvg server updating rule with Adam/Yogi/Adagrad updating rules. We also include FedAMSGrad \citep{wang22adaptive} which follows exactly the same logic in Algorithm \ref{fed_adaptive_alg}. \cite{reddi2020adaptive} further provides convergence analysis for FedAdam/FedYogi/FedADAGrad in general nonconvex settings and demonstrates strong empirical performances in both vision and language benchmarks compared to FedAvg and FedAvgM. However, their theoretical analysis relies on a key assumption that is $\beta_1=0$, i.e. there is no momentum, which rarely holds in reality. \cite{wang22adaptive} gets away with the $\beta_1=0$ requirement and provides convergence analysis of FedAMSGrad and FedAMSGrad with compression. Both \citep{reddi2020adaptive} and \citep{wang22adaptive} only consider synchronous aggregation and identical steps of local computation across devices.

To study the interplay between adaptive server optimization and system heterogeneity, we propose Autonomous Federated Adaptive Optimization, as is shown in Algorithm \ref{alg:autonomous_fed_algs}. For expository purposes, we only provide the pseudocode of Autonomous FedAdagrad. The extension to Autonomous FedAdam/FedAMSGrad/FedYogi is straightforward.

==> subfiles/scratch.tex <==
\iffalse

\begin{figure*}[h]
\vspace*{-12pt}
\centering
\subfigure[Training Curves]{
\hspace{0pt}
\includegraphics[width=.35\textwidth]{figs/cifar10_resnet_adaptive_delay_5_niid_3_train.eps}
\label{subfig:cifar10_resnet_adaptive_delay_5_niid_3_train}
}
\subfigure[Testing Curves]{
\hspace{0pt}
\includegraphics[width=.35\textwidth]{figs/cifar10_resnet_adaptive_delay_5_niid_3_test.eps}
\label{subfig:cifar10_resnet_adaptive_delay_5_niid_3_test}
}
\vspace*{-6pt}
\caption{Training and testing curves for various CC-Federated Adaptive Optimizers (ResNet on CIFAR-10) Concentration Parameter = 3.0.}
\label{fig:cifar10_resnet_adaptive_delay_5_niid_3_result}
\end{figure*}

\vspace*{5pt}
\noindent\textbf{Improvement is Consistent under Various Settings}
\vspace*{5pt}

\fi


\iffalse

\begin{figure*}[h]
\vspace*{-12pt}
\centering
\subfigure[Training Curves]{
\hspace{0pt}
\includegraphics[width=.35\textwidth]{figs/cifar10_resnet_adaptive_delay_5_train.eps}
\label{subfig:cifar10_resnet_adaptive_delay_5_train}
}
\subfigure[Testing Curves]{
\hspace{0pt}
\includegraphics[width=.35\textwidth]{figs/cifar10_resnet_adaptive_delay_5_test.eps}
\label{subfig:cifar10_resnet_adaptive_delay_5_test}
}
\vspace*{-6pt}
\caption{Training and testing curves for various CC-Federated Adaptive Optimizers (ResNet on CIFAR-10) Concentration Parameter = 0.5.}
\label{fig:cifar10_resnet_adaptive_delay_5_result}
\end{figure*}

\fi


\begin{figure}[h]
\vspace*{-12pt}
\centering
\subfigure{
\hspace{0pt}
\includegraphics[width=.32\textwidth]{figs/cifar10_resnet_adaptive_delay_10_test.eps}
}
\vspace*{-12pt}
\caption{Testing curve for various CC-Federated Adaptive Optimizers (ResNet on CIFAR-10) with maximum random delay $\tau=10$.}
\vspace*{-6pt}
\label{fig:cifar10_resnet_adaptive_delay_10_test}
\end{figure}



\begin{figure}[h]
\vspace*{-12pt}
\centering
\subfigure{
\hspace{0pt}
\includegraphics[width=.32\textwidth]{figs/fmnist_simple_cnn_adaptive_delay_10_niid_03_test.eps}
}
\vspace*{-12pt}
\caption{Testing curve for a CNN architecture on Fashion-MNIST.}
\vspace*{-6pt}
\label{fig:fmnist_simple_cnn_adaptive_delay_10_niid_03_test}
\end{figure}
